Conclusion Stability for Natural Language Based Mining of Design Discussions

Developer discussions range from in-person hallway chats to comment chains on bug reports. Being able to identify discussions that touch on software design would be helpful in documentation and refactoring software. Design mining is the application of machine learning techniques to correctly label a given discussion artifact, such as a pull request, as pertaining (or not) to design. In this paper we demonstrate a simple example of how design mining works. We then show how conclusion stability is poor on different artifact types and different projects. We show two techniques -- augmentation and context specificity -- that greatly improve the conclusion stability and cross-project relevance of design mining. Our new approach achieves AUC of 0.88 on within dataset classification and 0.80 on the cross-dataset classification task.

==> saner_sections/01-introduction.tex <==
\section{Introduction}
\label{sect:introduction}

Design discussions are an important part of software development. Software design is a highly interactive process and many decisions involve considerable back and forth discussion. These decisions greatly impact software architecture \cite{Kazman2016,woods16}.
%\footnote{``Software architecture is the set of design decisions, which, if made incorrectly, may cause the your project to be cancelled (https://twitter.com/danielbryantuk/status/1092823367021932544)''} 
However, software design is a notoriously subjective concept. For the related term `software architecture', for example, the Software Engineering Institute maintains a list of over 50 different definitions \cite{Software-Engineering-Institute:2010aa}). This subjectivity makes analyzing design decisions difficult \cite{Shahbazian2018}. Researchers have looked for ways in which design discussions could be automatically extracted from different types of software artifacts \cite{Brunet2014,Shakiba2016,Alkadhi2017,Motta2018,Zanaty2018,Viviani2018b,Viviani2019}. This automatic extraction, which we call \emph{design mining}, is a subset of research based on mining software repositories. The potential practical relevance of research on design mining include supporting design activities, improving traceability to requirements, enabling refactoring, and automating documentation.

A design mining study uses a corpus consisting of \emph{discussions}, in the form of software artifacts like pull requests, and manually labels those discussions targeting design topics, according to a coding guide. Machine learning classifiers such as support vector machines learn the feature space based on a vectorization of the discussion, and are evaluated using the gold set with metrics like area under the ROC curve.%, precision, and recall.

Producing a good-performing, validated classifier has been the main objective to date for design mining research. Apart from a validation study in Viviani et al. \cite{Viviani2019}, however, the practical relevance (cf. \cite{Oliveira-Neto:2019aa}) of design mining has not been studied in detail. Practical relevance in the context of design mining means a classifier with broad applicability to different design discussions, across software projects and across artifact types. Our goal is a practically relevant classifier, which we could run on a randomly selected Github project and identify with high accuracy that project's design discussions. 

Practical relevance can be seen as a form of external validity or generalizability, and the underlying concept is \emph{conclusion stability}, after Menzies and Sheppherd \cite{Menzies2012}. 
Design mining research has to date performed poorly when applied to new datasets (which we elaborate on in a discussion of related work, following). 
This is problematic because positive, significant results in a single study are only of value if they lend confidence to scientific conclusions. 
Conclusion stability, and a researcher's confidence they have found a true effect, relies on the ability to transfer a learner from an initial dataset (given the choices above) to other datasets, which may or may not match the initial study conditions.
To gain more insight on the challenges of conclusion stability in design mining, we report on two research objectives.



==> saner_sections/02-background-related-work.tex <==
\section{Background and Related Work}
\label{sect:related_work}

Our paper brings together two streams of previous research. First,  we highlight work on transfer learning in software engineering.
Secondly, we discuss previous work in mining design discussions and summarize existing results as an informal meta-analysis.

\subsection{Cross-Project Classifiers in Software Engineering}
A practically relevant classifier is one that can ingest a text snippet---design discussion---from a previously unseen software design artifact, and label it \textsf{Design/Not-Design} with high accuracy. 
Since the classifier is almost certainly trained on a different set of data, the ability to make cross-dataset classifications is vital. 
Cross-dataset classification \cite{Zimmermann:2009} is the ability to train a model on one dataset and have it correctly classify other, different datasets. 

The challenge is that the underlying feature space and distribution of the new datasets differ from that of the original dataset, and therefore the classifier often performs poorly. 
For software data, the differences might be in the type of software being built, the size of the project, or how developers report bugs.
To enable cross-domain learning without re-training the underlying models, the field of transfer learning applies machine learning techniques to improve the transfer between feature spaces \cite{Pan:2010}. Typically this means learning the two feature spaces and creating mapping functions to identify commonalities.

A related concept is the notion of \emph{conclusion stability} from Menzies and Sheppherd \cite{Menzies2012}. 
Conclusion stability is the notion that an effect X that is detected in one situation (or dataset) will also appear in other situations. 
Conclusion stability suggests that the theory that predicts an effect X holds (transfers) to other datasets. In design mining, then, conclusion stability is closely tied to the ability to transfer models to different datasets.

%That led to work on the problem with bias and variance in sampling for software engineering studies \cite{Kocaguneli2013}, where Menzies and first author Kocaguneli concluded that perhaps this tradeoff is not as important in software studies\footnote{from \cite{Menzies2012}, where $S$ is a study accuracy statistic, and $\hat{S}$ is the population (true) statistic: ``bias is $S - E(\hat{S})$ where $E$ is the expected value and the variance is $E((S - \hat{S})^2)$"}. 

There have been several lines of research into transfer learning in software engineering. We summarize a few here. 
Zimmermann et al. \cite{Zimmermann:2009} conducted an extensive study of conclusion stability in defect predictors. 
Their study sought to understand how well a predictor trained with (for example) defect data from one brand of web browser might work on a distinct dataset from a competing web browser. 
% The lessons from this paper were presented recently as part of a most-influential ten year retrospective. 
Only 3.4\% of cross-project predictions achieved over 75\% accuracy, suggesting transfer of defect predictors was difficult. 

Following this work, a number of other papers have looked at transfer learning within the fields of effort estimation and defect prediction. Sharma et al \cite{Sharma:2019aa} have applied transfer learning to the problem of code smell detection. 
They used deep learning models and showed some success in transferring the classifier between C\# and Java. However, they focus on source code mining, and not natural language discussions. Code smells, defect prediction, or effort estimation are quite distinct from our work in design discussion, however, since they tend to deal with numeric data, as opposed to natural language.

Other approaches include the use of bellwethers \cite{Krishna:2016:TMA:2970276.2970339}, exemplar datasets that can be used as simple baseline dataset for generating quick predictions. The concept of bellwether for design is intriguing, since elements of software design, such as patterns and tactics, are generalizable to many different contexts.

As far as we know, there has not been any use of transfer learning in natural language processing tasks for software engineering beyond the early results of Robbes and Janes \cite{Robbes:2019}, who reported on using ULMFiT \cite{Howard:2018} for sentiment analysis. We also use the transfer NLP potential of ULMFiT, which we discuss in \cite{Mahadi_2020}. Robbes and Janes emphasized the importance of pre-training the learner on (potentially small) task-specific datasets. We extensively investigate the usefulness of this approach with respect to design mining.


\subsection{Mining Design Discussions}
\label{sec:related_mining}
%This covers what the Viviani and Brunet papers were doing, as well as the more general question of design discussion.
While repository mining of software artifacts has existed for two decades or more, mining repositories for \emph{design-related} information is relatively recent. In 2011 Hindle et al. %and the second author of this paper, Ernst, 
proposed labeling non-functional requirements in order to track a project's relative focus on particular design-related software qualities, such as maintainability \cite{hindle11msr}. Hindle later extended that work \cite{HindleBZN15} by seeking to cross-reference commits with design documents at Microsoft. Brunet et al. \cite{Brunet2014} conducted an empirical study of design discussions, and is the target of our strict replication effort. They pioneered the classification approach to design mining: supervised learning by labeling a corpus of design discussions, then training a machine learning algorithm validated using cross-validation. 

In Table \ref{table:related} we review some of the different approaches to the problem, and characterize them along the dimensions of how the study defined ``design'', how prevalent design discussions were, what projects were studied, and overall accuracy for the chosen approaches. We then conduct a rudimentary vote-counting meta-review \cite{Pickard1998} to derive some overall estimates for the feasibility of this approach (final row).

\begin{table*}
    \centering
        \caption{\small{Comparison of recent approaches to design discussion detection. Effectiveness captures the metric the paper reports for classifier effectiveness (accuracy, precision, recall, F1). NB: Naive Bayes; LR: Logistic Regression; DT: Decision Tree; RF: Random Forest; SVM: Support Vector Machine}} 
        \label{table:related}
%    \rowcolors{2}{gray!25}{white}
%    \noindent\begin{tabularx}{300px}{c|c|c|c|c|X|X|X}
    \begin{tabular}{cp{1.4cm}p{1.4cm}p{1.2cm}p{1.4cm}p{1.2cm}p{2.7cm}p{2.4cm}}
    %\begin{tabular}{c|p{1.4cm}|p{1.4cm}|p{1.2cm}|p{1.4cm}|p{1.2cm}|p{2.4cm}|p{2.4cm}}
        \toprule
%        \rowcolor{gray!50}
    \textbf{Study} &  \textbf{Projects Studied} & \textbf{Data Size} & \textbf{ML Algorithm} & \textbf{Effectiveness} & \textbf{Prevalence} & \textbf{Defn. of Design} & \textbf{Defn. of Discussion}\\ 
    \midrule
    Brunet \cite{Brunet2014} & 77 high importance Github projects & 102,122 comments  & NB DT & \textbf{Acc: 0.86/0.94} & 25\% of discussions & design is the process of discussing the structure of the code to organize abstractions and their relationships. & A set of comments on pull requests, commits, or issues\\ 
    Alkadhi17 \cite{Alkadhi2017}  & 3 teams of undergrads & 8,702 chat messages of three development teams & NB SVM + undersampling & \textbf{Prec: 0.85} & 9\% of messages & Rationale captures the reasons behind decisions. & Messages in Atlassian HipChat\\ 
    Alkadhi18 \cite{Alkadhi2018} & 3 Github IRC logs & 7500 labeled IRC messages & NB SVM & \textbf{Prec. 0.79} & 25\% of subset labeled & Rationale captures the reasons behind decisions. & IRC logs from Mozilla\\ 
    Zanaty \cite{Zanaty2018}  & OpenStack Nova and Neutron & 2817 comments from 220 discussions & NB  SVM KNN DT & \textbf{Prec: 0.66 Recall: 0.78} & 9-14\% & Brunet's \cite{Brunet2014} & Comments on code review discussions\\ 
    Shakiba \cite{Shakiba2016}  & 5 random Github/SF & 2000 commits & DT  RF NV  KNN & \textbf{Acc: 0.85} & 14\% of commits & None. & Commit comments\\ 
    Motta \cite{Motta2018}  & KDELibs & 42117 commits, 232 arch & Wordbag matching & n/a & 0.6\% of commits & Arch keywords from survey of experts & Commit comments\\ 
    Maldonado \cite{Maldonado2017} & 10 OSS Projects & 62,566 comments & Max Entropy & \textbf{F1: 0.403 } & 4\% design debt & Design Debt: comments indicate that there is a problem with the design of the code & Code comment\\ 
    Viviani18 \cite{Viviani2018} & Node, Rust, Rails & 2378 design-related paragraphs & n/a (qualitative) & n/a & 22\% of paragraphs & A piece of a discussion relating to a decision about a software system’s design that a software development team needs to make & Paragraph, inside a comment in a PR\\
    Viviani19 \cite{Viviani2019} & Node, Rust, Rails & 10,790 paragraphs from 34 pull requests & RF & \textbf{AUC 0.87} & 10.5\% of paragraphs & same as Viviani18 & same as Viviani18\\
    Our previous paper \cite{Mahadi_2020} & StackOverflow discussions & 51,990 questions and answers & LR/ SVM/ ULMFiT & \textbf{AUC: 0.84} & n/a  & A question or answer with the tag ``design" & StackOverflow question/answer \\ %(36,425 design questions)
    (This paper) & StackOverflow discussions and literature & 260000 questions, answers and comment; corpus built from 300 literature of software engineering containing 1575439 total words with 20607 unique words  & kNN/ DT/ RF/ LR/ GNB/ NN/ AdaBoost/ QDA/ LSVM/ RBF SVM & \textbf{AUC: 0.80 with cross data (new state-of-the-art)} & n/a  & Stackoverflow questions with tags related to ``design" & StackOverflow question/answer/comments \\
     \midrule
    Meta & Open-source & 29,298 & n/a &\textbf{Acc: 0.85-0.94} & 13.78\% & n/a & n/a \\ %230,202 / 8 =  108.6 / 8
        \bottomrule
\end{tabular}
\end{table*}
    
\noindent\textbf{Defining Design Discussions}---The typical unit of analysis in these design mining studies is the ``discussion'', i.e., the interactive back-and-forth between project developers, stakeholders, and users. As Table \ref{table:related} shows, this changes based on the dataset being studied. A discussion can be code comments, commit comments, IRC or messaging application chats, Github pull request comments, and so on. The challenge is that the nature of the conversation changes based on the medium used; one might reasonably expect different discussions to be conducted over IRC vs a pull request.

\noindent\textbf{Frequency of Design Discussions}---Aranda and Venolia \cite{Aranda_2009} pointed out in 2009 that many software artifacts do not contain the entirety of important information for a given research question (in their case, bug reports). Design is, if anything, even less likely to appear in artifacts such as issue trackers, since it operates at a higher level of abstraction. Therefore we report on the average prevalence of design-related information in the studies we consider. On average 14\% of a corpus is design-related, but this is highly dependent on the artifact source. 
    
\noindent\textbf{Validation Approaches for Supervised Learning}---In Table \ref{table:related} column \textsf{Effectiveness} reports on how each study evaluated the performance of the machine learning choices made. These were mostly the typical machine learning measures: accuracy (number of true positives + true negatives divided by the total size of the labeled data), precision and recall (true positives found in all results, proportion of results that were true positives), and F1 measure (harmonic mean of precision and recall). 
Few studies use more robust analyses such as AUC (area under ROC curve, also known as balanced accuracy, defined as the rate of change). 
Since we are more interested in design discussions, the minority class of the dataset, AUC or balanced accuracy gives a better understanding of the result, because of the unbalanced nature of the dataset.

\noindent\textbf{Qualitative Analysis}
The qualitative approach to design mining is to conduct what amount to targeted, qualitative assessments of projects. The datasets are notably smaller, in order to scale to the number of analysts, but the potential information is richer, since a trained eye is cast over the terms. The distinction with supervised labeling is that these studies are often opportunistic, as the analyst follows potentially interesting tangents (e.g., via issue hyperlinks). Ernst and Murphy \cite{Ernst:2012wf} used this case study approach to analyze how requirements and design were discussed in open-source projects. One follow-up to this work is that of Viviani, \cite{Viviani2018,Viviani2019}, papers which focus on rubrics for identifying design discussions. The advantage to the qualitative approach is that it can use more nuance in labeling design discussions at more specific level; the tradeoff of course is such labeling is labour-intensive. 

\noindent\textbf{Summary}
A true meta-analysis \cite{Pickard1998,Kitchenham2019} of the related work is not feasible in the area of design mining. 
Conventional meta-analysis is applied on primary studies that conduct experiments in order to support inference to a population, which is not the study logic of the studies considered here. 
For example, there are no sampling frames or effect size calculations. 
One approach to assessing whether design mining studies have shown the ability to detect design is with vote-counting (\cite{Pickard1998}), i.e., count the studies with positive and negative effects past some threshold. 

As a form of vote-counting, the last row of Table \ref{table:related} averages the study results to derive estimates. 
On average, each study targets 29,298 discussions for training, focus mostly on open-source projects, and find design discussions in 14\% of the discussions studied. 

As for effectiveness of the machine learning approaches, here we need to define what an `effective' ML approach is. 
Since this is a two label problem a random guessing approach on a balanced dataset would achieve accuracy of 50\%. Balanced accuracy, defined as ( true negative rate + true positive rate )/2, will always be 50\% for a random guesser in the 2 label case. 
Since balanced accuracy is equivalent to AUC, we see that only our previous paper \cite{mahadi20} and Viviani's work \cite{Viviani2019} perform well. While the other papers report reasonable scores for F1, Accuracy, and Precision, none of them balance their data, so their imbalanced datasets mean the results are significantly higher than a balanced dataset would support. 


%For our purposes, we can objectively define this as ``outperforms a baseline ZeroR learner". 
% The ZeroR learner labels a discussion with the majority class, which is typically ``non-design". 
% In a balanced, two label dataset, the ZeroR learner would therefore achieve accuracy of 50\%. 
% In an unbalanced dataset, which is the case for nearly all design mining studies, ZeroR is far more `effective'. Using our overall average of 14\% prevalence, a ZeroR learner would achieve accuracy of $(1-0.14) = 0.86$. 
% This is the baseline for accuracy effectiveness. 
% For precision and recall, ZeroR would achieve 0.86 and 1, for an F1 score of 0.93. 
% Comparing this baseline to the studies above, we find that only Brunet and our approach below surpass this baseline. In other words, few studies are able to supersede random, majority-class labeling.


==> saner_sections/04-cross-dataset-comparison.tex <==
\begin{table*}[h]
 \centering
 \caption{Datasets used for within and cross-dataset classification. All datasets are English-language}
 \label{tbl:newdatasets}
 \begin{tabular}{ccp{1.8cm}p{1cm}p{1cm}p{2.4cm}p{1.4cm}p{1.4cm}}  \toprule
 \textbf{Citation} & \textbf{Dataset} & \textbf{Type}  & \textbf{Total instances} & \textbf{Design instances} & \textbf{Projects} & \textbf{Mean Discussion Length (words) } & \textbf{Vocabulary Size (words)} \\
 \midrule
 \cite{Brunet2014} & Brunet 2014  &  Pull requests & 1,000 & 224 & BitCoin, Akka, OpenFramework, Mono, Finagle & 16.97 & 3,215 \\
\cite{Shakiba2016} & Shakiba 2016  & Commit messages & 2,000 & 279 & Random Github and SourceForge  & 7.43 & 4,695 \\
 \cite{Viviani2018} & Viviani 2018   &   Pull requests & 5,062 & 2,372 & Node, Rust, Rails & 36.13 &  24,141 \\
\cite{Maldonado2017} & SATD  & Code comments & 62,276 & 2,703 & 10 Java incl Ant, jEdit, ArgoUML & 59.13 & 49,945 \\ %4070 
self & StackOverflow & StackOverflow questions & 51,989 & 26,989 & n/a & 114.79 & 252,565 \\
 \bottomrule
 \end{tabular}
 \end{table*}
 
 
 \section{Research Objective 2: Conclusion Stability}
\label{sect:conclusion_s}
In this section we build on the replication results and enhancements of our first research objective. We have a highly accurate classifier, NewBest, that does well \emph{within-dataset}. We now explore its validity when applied to other datasets, i.e., whether it has conclusion stability. 

In \cite{Menzies2012}, Menzies and Shepperd discuss how to ensure conclusion stability. They point out that predictor performance can change dramatically depending on dataset (as it did in Zimmermann et al. \cite{Zimmermann:2009}). Menzies and Shepperd specifically analyze prediction studies, but we believe this can be generalized to classification as well. Their recommendations are to a) gather more datasets and b) use train/test sampling (that is, test the tool on different data entirely). 

In this section we evaluate a classifier trained on one dataset to a different dataset, but consisting of the same types of discussions. Before beginning to apply learners to different datasets, it makes sense to ask if this transfer is reasonable. For example, in Zimmermann et al. \cite{Zimmermann:2009} the specific characteristics of each project were presented in order to explain the intuition behind transfer. 
E.g., should a discussion of design in StackOverflow be transferable, that is, considered largely similar to, one from Github pull requests? 

 
\subsection{Research Method}
In Table \ref{tbl:newdatasets} we illustrate each of the datasets considered in this paper. In Table \ref{tbl:examples} we show some sample design discussions from each.
Since performance of transfer learning is largely based on similarity between projects (i.e., feature spaces), we would expect to see better AUC results for cross-project prediction if data sources are the same (e.g. pull requests), projects are the same, and/or the platforms are the same (e.g. Github). 

We test the ability to transfer classifiers to new types of discussions and datasets.
%We report results in Fig. \ref{fig:cross_project_validation}. There we show only AUC scores for the transferred learner of 0.65 AUC or greater. \neil{why 65?}
We applied the best protocol result from above. That is, the NewBest classifier, using \textsf{stopwords+oversampling+TF-IDF+Logistic Regression}. 
% We use the classifier with data from totally different datasets. 
We train this classifier on the Brunet \cite{Brunet2014} data, and the other 4 datasets described in Table \ref{tbl:newdatasets}.

We then apply the trained model, as well as the ULMFiT model described below, to each dataset in turn (thus, 5 comparisons, including within-project labeling for a baseline).
%we apply it to self-admitted technical debt (SATD) \cite{Maldonado2017}, which are code comments labeled as design-related technical debt or other sources of technical debt,and a dataset we created based on StackOverflow questions tagged design (see discussion in \S \ref{sec:doc2vec} above).

 \begin{table}[htb]
 \centering
 \caption{Sample (raw) design discussions, pre data cleaning.}
 \label{tbl:examples}
 \begin{tabular}{cp{6.2cm}} 
 \toprule
 \textbf{Dataset} & \textbf{Sample Snippet}  \\
 \midrule
StackOverflow & \emph{What software do you use when designing classes and their relationship, or just pen and paper?} \\
Brunet 2014 & \emph{Looks great Patrik Since this is general purpose does it belong in util Or does that introduce an unwanted dependency on dispatch} \\
SATD & \emph{// TODO: allow user to request the system or no parent}\\
Viviani 2018 & \emph{Switching the default will make all of those tutorials and chunks of code fail with routing errors, and ``the RFC says X" doesn't seem like anywhere near a good enough reason to do that.} \\
Shakiba 2016 & \emph{Move saveCallback and loadCallback to RequestProcessor class } \\
 \bottomrule
 \end{tabular}
 \end{table}

\subsection{Transfer Learning with ULMFiT}
\label{sec:ulmfit}
Early results reported by Robbes and Janes \cite{Robbes:2019} suggested recent work on ULMFiT (Universal Language Model Fine-Tuning, \cite{Howard:2018}) might work well for transfer learning in NLP for the software domain. They applied it to the task of sentiment analysis. 

 ULMFiT uses a three layer bi-LSTM (long short-term memory) architecture. It supports transfer learning for NLP tasks without having to train a new model from the beginning. ULMFiT uses novel NLP techniques like discriminative fine tuning, gradual unfreezing and slanted triangular learning rates which makes it state-of-the-art \cite{Howard:2018}. 
 ULMFiT comes pre-trained using data on a Wikipedia dataset. Wikipedia lacks software specificity.
 Our aim using ULMFiT was to observe the behavior of the pre-trained ULMFiT model (AWD-LSTM) when we train its last neural network layer with the Stack Overflow design discussion data. The StackOverflow data fine-tunes the contextual layers of the model.
 We combined the Stack Overflow data along with the four design-specific datasets for training. 

For our ULMFiT deep learning (DL) approach we used the DL practice \cite{James2013} of a 60\%-20\%-20\% train-validate-test ratio, where the test set is held back from training and validation. We ran this 3 times and noticed only trivial changes (less than 0.5\%) in the results for any of the runs. We report the mean.

We had two reasons for this choice. First, the anticipated training costs and data size are much larger in deep network models. Second, we wanted to test the claimed capability of ULMFiT \cite{Howard:2018} to performs well on small sample sizes (60\% of our dataset). Unsurprisingly, adding more data points increases performance, at the cost of overfitting (detailed results can be found in our replication package).

Fine-tuning ULMFiT incorporates internal error assessment using a validation and train loss technique to determine the optimal trained model by constantly observing the difference between train loss and validation loss. %If the validation loss is greater than train loss, then the model starts overfitting and vice versa. Fig. \ref{fig:Lossplot} shows this train and validation loss. 
This informs model selection, which is then tested against the held-back test set.

Training ULMFiT involves first, model pre-training using the AWD-LSTM state of the art language modelling technique; second, fine tuning the learning rate of the language model to get the optimal value of learning rate. This can be done per layer of the neural network.
% We can go deeper into the neural network layers of the AWD-LSTM and fine tune each layer as required by keeping in mind on every step that the model does not overfit or underfit.

In the third stage, train the language classification model on top of a pre-trained language learner model. The training data remains StackOverflow, but now in the supervised, design-labeled context. Finally, we again fine-tune our trained text classifier learner to find an optimal learning rate to gain a good balance between overfitting and underfitting the model. For this experiment, our optimal learning rate was 0.01. %Again, we can unfreeze the pre-trained LSTM layers and go deeper to fine tune each layer in order to get much higher predicting performance and run more epochs to achieve further fine tuned result.

After performing the above steps by combining the StackOverflow dataset---questions tagged design/non-design---and the Brunet2014 dataset, AUC was approximately 93\% during the training phase (i.e., within sample performance).
To ensure the model is not overfitting or underfitting, we plot the recorded train and validation losses. 
We make sure that the train and validation losses are close to each other. 
Fig. \ref{fig:Lossplot} is the result after 3 epochs of model training with the learning rate of 0.01, which is the optimal learning rate for this model. 
We see that the training loss is close to the validation loss (0.18 vs 0.22). 
This suggests the trained model is performing well. %After further fine tuning and running more epochs, there is a possibility that we may get the training loss more closer to the validation loss.

%While training deep neural networks, performing cross-validation techniques can be challenging in terms of the time required to train on each fold of data especially when the training data is huge (StackOverflow data in this case). 
%The method we chose to identify the efficiency of the predictive model was by visualizing the difference between the train loss and validation loss.
%\neil{could drop the previous para}

\begin{figure}[hbt]
\centering
  \includegraphics[width=0.35\textwidth]{fig/ulmfit/loss_plot_3_epochs.JPG}
  \caption{Loss plot after 3 epochs}
  \label{fig:Lossplot}
\end{figure}

 \begin{figure*}[hbt]
  \begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{fig/heatmap_newbest.png}
  \caption{NewBest results.}
  \label{fig:sfig1}
\end{subfigure}
  \begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{fig/heatmap_ulm_new.png}
  \caption{ULMFiT results. }
  \label{fig:sfig2}
\end{subfigure}
\caption{Cross-dataset design mining. Numbers: AUC. Read these plots as ``the model trained on the Dataset  on the X axis has AUC \emph{value} Tested On Dataset on the Y Axis". Higher intensity = better score.}
\label{fig:cross-results}
\end{figure*}
%
%The results in Table \ref{tbl:newdatasets} highlight the results after performing transfer learning using ULMFiT on the other datasets. Our model 'Stackoverflow Dataset + Combined Dataset in \cite{Viviani2018}' was trained only using the vocabulary present in both the datasets and the same was for 'Stackoverflow Dataset + Combined Dataset in \cite{Brunet2014}'. While performing transfer learning, the model predictions were based on the Vocabulary on which it was trained. While analyzing the dataset, we observed that although the design discussions were in natural language, there were many words that were unique to the open source technology. We observed that the more vocabulary we feed to our ULMFiT model, the more it knows and gets tuned on the language modelling resulting in better classification. Although, the results are just slightly improved only in some cases compared to our previous approach, 

Our current approach is trained using a LSTM Neural Network. This indicates there is also scope for fine-tuning several layers of the neural network in order to gain better performance on predictions. 

\subsection{Results}
Results are summarized in the heat maps shown in Fig.  \ref{fig:cross-results}. More intense color is better. On the left, Fig. \ref{fig:sfig1} shows the results for the NewBest protocol (SVM with word embeddings). On the right, Fig \ref{fig:sfig2} shows the equivalent for the ULMFiT approach. Our replication package includes complete results including confidence intervals and tests of significance.

The main challenge for conclusion stability with design mining datasets is that it is hard to normalize natural language text. 
This means while two datasets might reasonably be said to deal with design, one might have chat-like colloquial sentences, while the other has terse, template-driven comments.  We illustrate this difference with the example discussions shown in Table \ref{tbl:examples}.
In comparing to other datasets the comparison should still be over reasonably similar `apples'. As Table \ref{tbl:newdatasets} shows, there is some variance in all five datasets, with the type of discussion artifact, source projects, and linguistic characteristics differing. However, despite these differences Table \ref{tbl:examples} suggests there should be broad similarities: e.g., concepts such as \texttt{Class} or \texttt{User}, or ideas like moving functionality to different locations. Intuitively, we suggest the notion of transfer ought to work to some extent on these datasets: they are not completely different.

For the NewBest approach, the diagonal starting bottom-left captures the \emph{within-dataset} performance, which as expected, is better than the cross-dataset AUC scores. Secondly, all models performed best on the Brunet test dataset (bottom row). This is because in building the NewBest classifier, we evaluated our protocol choices against the Brunet dataset. This shows how tightly coupled protocol choices and conclusion stability are.

It also seems to be the case that results are poorer for datasets that are more removed from each other: using pull requests (Viviani and Brunet) does little better than random for StackOverflow and code comments (SATD).

For the ULMFiT results in Fig. \ref{fig:sfig2}, we can see the benefit of training with the StackOverflow dataset plus the fine-tuning (i.e., each tic on the x-axis reflects the fine-tuning in addition to StackOverflow training). This is shown by the good results in the top row, which are essentially within-dataset results. Other results, however, are poor, and particularly when compared to the NewBest results (which is also quicker to train). A Kruskal-Wallis test of significance shows no differences between the two learners. We therefore do not see much benefit from the way we have applied ULMFiT for cross-dataset classification of design. 

We ran 10-fold cross-validation on ULMFiT as well, and report those results in the replication package. For the transfer learning research objective, ten fold validation does not make a significant difference in AUC. Transfer performance on Brunet2014 data only changes from 0.502 to 0.588, even with the additional data. Thus, our conclusion that ULMFiT is not a significant improvement on the transfer learning problem remains the same.

Although the design discussions were in natural language, there were many words that were unique to the software/open source domain. We observed that the more vocabulary we feed to our ULMFiT model, the more it knows, the more it gets tuned on the language modelling, the better it performed. Thus we see great benefit in increasing the software-specific, dataset agnostic data we train ULMFiT.

==> table_summary.tex <==
\begin{table}[!ht]
\caption{Tabular form of Figures \ref{fig:we_comparison}, \ref{fig:similar_wi_a} and \ref{fig:similar_wi_b}. Here,  KNN = Nearest Neighbor, DT = Decision Tree, RF = Random Forrest, LR = Logistic Regression, GNB = Gaussian Naive Bayes, NN = Neural Net, AB = Ada Boost, QDA = Quadratic Discriminant Analysis, LSVM = Linear Support Vector Machine, RBF SVM = Radial Basis Function Support Vector Machine.}
\label{tab:result-table}
\centering
\begin{tabular}{p{0.2\textwidth}|p{0.05\textwidth}|p{0.03\textwidth}|p{0.03\textwidth}|p{0.03\textwidth}|p{0.04\textwidth}|p{0.03\textwidth}|p{0.03\textwidth}|p{0.04\textwidth}|p{0.06\textwidth}|p{0.05\textwidth}}
\toprule
Reference data in the figure & KNN & DT     & RF  & LR  & GNB & NN  & AB  & QDA & LSVM & RBF SVM \\ \midrule
Figure \ref{fig:we_comparison} blue bars             & 0.5 & 0.51 & 0.5 & 0.5 & 0.5 & 0.5 & 0.5 & 0.5 & 0.5  & 0.54    \\ \hline
Figure \ref{fig:we_comparison} orange bars and figure \ref{fig:similar_wi_a} blue bars & 0.63  & 0.62 & 0.69 & 0.74 & 0.64 & 0.68  & 0.65 & 0.60 & 0.76 & 0.73  \\ \hline
Figure \ref{fig:similar_wi_a} orange bars and figure \ref{fig:similar_wi_a} blue bars & 0.68 & 0.51 & 0.64 & 0.77 & 0.51 & 0.61  & 0.69 & 0.5    & 0.79 & 0.71 \\ \hline
Figure \ref{fig:similar_wi_b} orange bars                        & 0.73 & 0.56 & 0.73 & 0.79 & 0.70 & 0.70 & 0.71 & 0.67  & 0.80 & 0.78 \\ \bottomrule
\end{tabular}
\end{table}


